RECS: Robust Graph Embedding Using Connection Subgraphs

The success of graph embeddings or node representation learning in a variety of downstream tasks, such as node classification, link prediction, and recommendation systems, has led to their popularity in recent years. Representation learning algorithms aim to preserve local and global network structure by identifying node neighborhood notions. However, many existing algorithms generate embeddings that fail to properly preserve the network structure, or lead to unstable representations due to random processes (e.g., random walks to generate context) and, thus, cannot generate to multi-graph problems. In this paper, we propose RECS, a novel, stable graph embedding algorithmic framework. RECS learns graph representations using connection subgraphs by employing the analogy of graphs with electrical circuits. It preserves both local and global connectivity patterns, and addresses the issue of high-degree nodes. Further, it exploits the strength of weak ties and meta-data that have been neglected by baselines. The experiments show that RECS outperforms state-of-the-art algorithms by up to 36.85% on multi-label classification problem. Further, in contrast to baselines, RECS, being deterministic, is completely stable.

==> 020problem.tex <==
\section{Problem Formulation} \label{sec:problem}
We formally define the problem of representation learning for large-scale information networks using connection subgraphs as follows:\\

\noindent \textbf{Information Network.} An information network is defined as a graph $G=(V,E)$, where $V$ represents the set of nodes connected together by a set of edges $E$. The weight of an edge $e \in E$ indicates the strength of the relation among the two nodes connected through that edge. If $G$ is undirected---i.e., social networks, then for any two nodes; say node $u$ and node $v$, $(u,v)=(v,u)$ and thus, $w_{uv}=w_{vu}$. However, if $G$ is directed---i.e.,citation networks, we have $(u,v) \ne (v,u)$, and thus, $w_{uv} \neq w_{vu}$.\\

\noindent \textbf{Learning Large-scale Network Representations.} Given a large-scale network; $G=(V,E)$, the problem of learning a graph $G$ node representations strives to preserve local and global network structure while mapping each node $v \in V$ from a high-dimensional feature space to a low-dimensional feature space $R^d$ using a mapping function, $f_G \colon V \to R^d$, where $d \ll |V|$.\\

\noindent \textbf{Connection Subgraph.} Since learning node representations aims to preserve network structure, state-of-the-art algorithms have employed various proximity metrics, such as \textit{first-order proximity}~\cite{goyal2017graph}, and \textit{second-order proximity}~\cite{goyal2017graph}, in order to preserve graph local and global structure, respectively. However, such metrics are not sufficient enough, therefore, here in this study, we harness the analogy with electrical circuits using connection subgraphs~\cite{faloutsos2004fast} to capture proximity at different levels between any two non-adjacent nodes. Connection subgraph is defined as a group of nodes connecting any two randomly-sampled non-adjacent nodes in a graph. The nodes in between are extracted from the graph in two phases using two different aspects: 1) \textit{Distance}: so that the closer the node to either one of the two nodes of interest, the higher the chance that the node will be extracted and included in the subgraph, and 2) \textit{Network flow (current)}: after the first level of extraction, an extra current-driven refinement process is employed in order to omit any remaining spurious regions in the first extracted subgraph.



==> 030method_old.tex <==
\section{Proposed Method: RECS }\label{sec:method}
In this section, we describe our proposed method, RECS, a completely deterministic algorithm (unlike previous works~\cite{perozzi2014deepwalk,grover2016node2vec,perozzi2016walklets} that employ random processes), which is capable of preserving local and global---beyond two hops---connectivity patterns. As shown in Fig.~\ref{fig:RECS}, it consists of two main steps: (1) Neighborhood definistion via connection subgraphs, and (2) Representation vector update. We discuss the two steps in Sections~\ref{subsec:step1} and~\ref{subsec:step2}, respectively.


\begin{figure*}[t!]
\includegraphics[width=0.9\textwidth]{Figures/RECS.png}
\centering
\setlength{\abovecaptionskip}{15pt plus 3pt minus 2pt}
%\vspace{-0.5cm}
\caption{A description of RECS algorithm neighborhood definition step main phases: (a) Neighborhood expansion of node $u$ through \textit{$n-hop$} neighbors to generate $N_E(u)$ on distance basis. node $z$ indicates the grounded universal sink node. (b) Neighborhood refinement of $N_E(u)$ to generate $N_R(u)$ on current basis.}
\label{fig:RECS}
\end{figure*}


% which is inspired by the  as shown in Figure~\ref{fig:RECS}. Our algorithm is largely inspired by the connection subgraph algorithm proposed in~\cite{faloutsos2004fast}.

\reminder{is this the best place for this paragraph? Saba: not sure, but, can we move it up towards the end of the related work? added table 1.} While RECS is largely inspired by the connection subgraph algorithm proposed in~\cite{faloutsos2004fast} (described in Section.~\ref{sec:related}), there are major adaptations for our proposed representation learning setting. Table~\ref{my-label} shows a qualitative comparison between the connection subgraph algorithm and RECS.
% In RECS, we implement major changes to the connection subgraph algorithm in a way that better serves our study objectives. This is rooted to the change in context that the original study~\cite{faloutsos2004fast} has been developed for. Technically-speaking, 
The heart of learning node representations is to obtain representative node neighborhoods, which preserve local and global connections simultaneously. %That is, good node neighborhoods should preserve local and global connections well. 
We find that connection subgraphs are beneficial in this setting, since they allow us to: (1) Better control the search space; (2) Benefit from actual flow, meta-data, that is being neglected by state-of-the-art algorithms; (3) Exploit the strength of weak ties; (4) Avoid introducing randomness caused by random/biased walks; (5) Integrate two extreme search strategies, breadth-first search (BFS) and depth-first search (DFS)~\cite{zhou2006breadth}; %, where immediate neighbors and neighbors at increasing distances from the pair of non-adjacent nodes---i.e., source and destination nodes---, are considered, respectively
(6) Address the issue of high-degree nodes; %, that is, a node with high-degree distribution has a low chance to be included in the connection subgraph, as a pair of nodes might be incidentally connected through a high-degree distribution node
and (7) Better handle non-adjacent nodes that are ubiquitous in real-world large-scale graphs.

\begin{table}[]
\ssmall
\centering
\caption{Qualitative comparison of the connection subgraph algorithm~\cite{faloutsos2004fast} vs. RECS.}
\label{my-label}
\begin{tabular}{@{}l|c|c@{}}
\hline
             & \textbf{Connection Subgraph}                 & \textbf{RECS}                                          \\ \hline
\textbf{Purpose}      & Node proximity (for only 2 nodes) & Neighborhood definition (for the whole graph) \\
\textbf{First step}  & Candidate generation (distance-driven)                & Neighborhood expansion (distance-driven)            \\
\textbf{Second step} & Display generation (delivered current-driven)                  & Neighborhood refinement (current-driven)                  \\
\textbf{Source}       & $u_i$                                & $u\: \forall \: u \in V$                              \\
\textbf{Target}       & $u_j$                                & Universal sink node $z$                         \\ \hline
\end{tabular}
\end{table}





% In contrast to previous works~\cite{perozzi2014deepwalk,grover2016node2vec,perozzi2016walklets}, which employ random walks to obtain node neighborhoods, and may result in unstable embeddings, we  propose RECS, a completely deterministic algorithm. RECS is also capable of preserving local and global---beyond two hops---connectivity patterns. It consists of two main steps: (1) Neighborhood definition, and (2) Representation vector update. We further discuss the two steps in Sections~\ref{subsec:step1} and~\ref{subsec:step2}, respectively.



\subsection{Step 1: Neighborhood Definition}
According to the analogy with electrical circuits, and by using the connection subgraph algorithm, we define node neighborhoods. The use of a subgraph instead of a single critical path between any two non-adjacent nodes is beneficial for several reasons: (1) Choosing the most important path using a fully automated mechanism is susceptible to errors; (2) Showing a subgraph elevates the probability of having the critical path, if present; and (3) The connection subgraph is better at characterizing the random spread of information in real-world networks than a single path. This step consists of two phases: (A) \textit{Neighborhood expansion}, and (B) \textit{Neighborhood refinement}. We provide an overview of each phase as follows:
\label{subsec:step1}

\vspace{0.15cm}
\noindent \textbf{Phase A: Neighborhood Expansion - $N_E(u)$.}
Before we explain the details of the \textit{neighborhood expansion} phase, we first highlight the prime difference between our study and original study~\cite{faloutsos2004fast} objectives. In~\cite{faloutsos2004fast}, the study aimed to capture the proximity among any two non-adjacent nodes at a time. Therefore, it implemented \textit{candidate generation} and \textit{display generation} phases, respectively. In the candidate generation phase, a distance-driven metric is employed to expand the neighborhoods of the two nodes until they ‘significantly’ overlap. In our study, on the other hand, we seek to generate neighborhood notion for each node in the graph. Although we generate neighborhood notions by capturing nodes proximities on the local and global levels, we still find~\cite{faloutsos2004fast} inefficient for our study context. That is,~\cite{faloutsos2004fast} only handles two nodes at a time, however, in our study, during any expansion process, we need to deal with the whole graph at one time. Thus, instead of implementing \textit{candidate generation}, here we propose to perform \textit{neighborhood expansion} phase. To this end, we introduce the universal sink node $z$ that is grounded ($V_z=0$). We connect node $z$ to all nodes in graph $G$, except node $u$, which we aim to expand. By that, we can capture proximities between node $u$ and all other nodes in $G$ during expansion. In addition, the introduction of node $z$ allows us to address the issue of high-degree nodes and exploit the strength of weak ties. It is worth mentioning that a pair of nodes is more likely to be incidentally connected together through a high-degree node---i.e., hop node.

Figure~\ref{fig:RECS}-a shows the expansion of node $u$'s neighborhood notion that includes a quick removal of nodes and edges that are too far from node $u$. Therefore, it generates a moderate-sized graph. Algorithm~\ref{Algorithm:1}-a shows the details of the \textit{expansion} process. %The \textit{expansion} subgraph is  treated as input to the \textit{refinement phase}.
Formally, the neighborhood \textit{expansion} process takes node $u$ in $G$ and starts to gradually and neatly expand its neighborhood on a distance basis. However, since we connect node $z$ to all nodes in $G$, we add a new edge to each node $n$ in $G$ (except node $u$). Node $n$ represents any node in graph, except node $u$. For that, we need to compute the edge weight between each node $n$ and node $z$, as shown in Eq.\eqref{eq:1}. Node $m$ represents any immediate neighbors of node $n$. $C(n,m)$ indicates the conductance or the weight of an edge between node $n$ and node $m$. $\alpha$ is a parameter we set to be $>0$. However, since this study handles unweighted graphs, we set $\alpha=1$. It is important to note that introducing node $z$ offers the opportunity to penalize high-degree nodes and accounts for the strength of weak ties. That is, a node with plenty of edges, the computed additional weight of the new edge with node $z$ would be relatively high.

The new graph---including the added node $z$ and its edges with graph $G$ nodes---is employed for distance computation using Eq.\eqref{eq:2} and Eq.\eqref{eq:3}. We employ Eq.\eqref{eq:2} for distance computations when node $n$ is an immediate neighboring node of node $u$. However, if node $n$ is not an immediate neighboring node of node $u$, we compute distance using Eq.\eqref{eq:3}. In Eq.\eqref{eq:3}, the first term, $\log (deg^{2}(u)/C^{2}(u,c))$, represents the distance from node $u$ to node $c$, where node $c$ is the closest immediate neighboring node to node $u$ that is connected to node $n$, and is already expanded before. The second term, $\log (deg^{2}(c)/C^{2}(c,n))$, represents the distance from node $c$ to node $n$. The numerator computations in Eq.\eqref{eq:2} and Eq.\eqref{eq:3} emphasize the fact that high-degree nodes are penalized in distance computations. In other words, a high-degree node would have high squared degree, where a node degree refers to the summation of weights incident to it. By that, it would appear farther during the \textit{expansion} process from node $u$. Therefore, it would be less probable to reveal in the \textit{expansion} subgraph.

\begin{equation} \label{eq:1}
\ssmall
\ C(n,z)=\alpha\sum_{m\neq z}C(n,m)
\end{equation}

\begin{equation} \label{eq:2}
\ssmall
\ Distance(u,n)=\log (deg^{2}(u)/C^{2}(u,n))
\end{equation}

\begin{equation} \label{eq:3}
\ssmall
\ Distance(u,n)=[\log (deg^{2}(u)/C^{2}(u,c))]+[\log (deg^{2}(c)/C^{2}(c,n))]
\end{equation}

After explaining the weight and distance computations, now we describe the way in which \textit{expansion} subgraph is generated. We define $EX$ as a set of expanded nodes. We initially set $EX$ to have node $u$. The expanded nodes are ultimately the nodes form the neighborhood \textit{expansion} subgraph. Likewise, let $P$ be the set of pending nodes that are to be expanded. $P$ is initially set to have node $u$'s immediate neighbors.
Now, that we have the set of pending nodes $P$, we expand by choosing the closest node to the root (source) of expansion, $u$, except node $z$. The selection of the closest node is based on the distance function shown in Eq.\eqref{eq:2} and Eq.\eqref{eq:3}. The intuition standing behind the \textit{expansion} process is that the closer the expanded node $n$ to the source node $u$, the lower information flow we lose. In order to capture proximity among any two non-adjacent nodes, it is always recommended to adopt the shortest path that maximizes the flow. The maximum flow that can pass through any edge would be the edge weight~\cite{faloutsos2004fast}. Once a node $n$ is expanded, we add its immediate neighbors to $P$, and we repeat the same process until we  have $|EX|=e$, where $e$ is a constant that represents the desired size of expanded subgraph. We show the \textit{neighborhood expansion} pseudocode in Algorithm~\ref{Algorithm:1}-a.

\vspace{0.15cm}
\noindent \textbf{Phase B: Neighborhood Refinement - $N_R(u)$.}
In this phase, as shown in Figure~\ref{fig:RECS}-b, we remove any remaining spurious regions in each \textit{expanded neighborhood} subgraph. The \textit{neighborhood refinement} phase takes an \textit{expanded} subgraph as an input and returns a \textit{refined neighborhood} subgraph as an output. The \textit{refined} subgraph is generated on a network flow (current) basis. Before we describe our \textit{refinement} process, we first highlight the change we make comparing to the original developed algorithm in~\cite{faloutsos2004fast}. In~\cite{faloutsos2004fast}, the second phase is the \textit{display generation}, which we instead call it the \textit{refinement} phase. In \textit{display generation}, delivered current  has been employed in order to prune out any remaining unrelated nodes in \textit{candidate generation} subgraph. It is important to note that the computations of `current' and `delivered current' are different. The computation of current is not as informative as delivered current, but is more efficient. The use of delivered current was not a major struggle in ~\cite{faloutsos2004fast}, because algorithm only processes one subgraph. However, on the contrary, we find the implementation of \textit{display generation} problematic for several reasons: 1) The large size of \tetxit{expanded} subgraph, $|N_E(u)|$; 2) The large size of \textit{refined} subgraph, $|N_R(u)|=800$, comparing to the \textit{display generation} subgraph size that is used to have a maximum of $30$ nodes; and 3) The extremely large number of subgraphs, $|V|$, that need to be processed, to ultimately generate node neighborhoods.

In order to refine \textit{expansion} subgraph, we perform \textit{neighborhood refinement} phase. In this phase, we link \textit{expansion} subgraph's nodes (output of $N_E(u)$), except source node $u$, to the previously introduced node $z$. We then start to gradually refining the \textit{expansion} subgraph on current-driven basis. The \textit{expansion} process includes adding an end-to-end path to the \textit{refined} empty subgraph until reaching specified \textit{refined} subgraph size, $|N_R(u)|$. The underlying intuition of the \textit{refinement} phase is to maximize the current reaches to node $z$ from the source node $u$. For that, we are required to calculate the current $I$ flows between any two immediate neighbors in the \textit{expanded} subgraph. In our context, $I$ indicates the meta-data or network flow that we aim to avail. We compute $I$ using Ohm's law. Based on Ohm's law shown in Eq.\eqref{eq:4}, in order for a current to flow from node $n_1$ to node $n_2$, we need node $n_1$ to have a higher voltage than node $n_2$, which is defied as the downhill constraint. $I(n_1,n_2)$ indicates the current flows from node $n_1$ to node $n_2$. $C(n_1,n_2)$ represents the conductance or the weight of the edge connecting node $n_1$ and node $n_2$. $V(n_1)$ and $V(n_2)$ indicate the voltages of node $n_1$ and node $n_2$, respectively. As presented by Ohm's law, in order to compute the currents between each two immediate nodes, we should first calculate their voltages. For voltage computations, we use Eq.\eqref{eq:5}. Node $n_i$ indicates any node in the \textit{expanded} subgraph, except nodes $u$ and $z$. Node $v$ represents an immediate neighboring node of node $n_i$, and $C(n_i,v)$ refers to the conductance (weight) of edge connects nodes $n_i$ and $v$. Most importantly, we compute any node $n_i$ voltage under the boundary conditions shown in Eq.\eqref{eq:6}. The nodes voltages are calculated by solving a system of linear equations.

\begin{equation} \label{eq:4}
\ssmall
I(n_1,n_2)=C(n_1,n_2)(V(n_1)-V(n_2))
\end{equation}

\begin{equation} \label{eq:5}
\ssmall
V(n_i)=\frac{\sum_{v}V(v)C(n_i,v)}{\sum_{v}C(n_i,v)} \eps\enspace \forall n\neq u,z
\end{equation}

\begin{equation}\label{eq:6}
\ssmall
 V(u)=1, V(z)=0
\end{equation}
%$v_j$: immediate neighbor of $u_i$}
%\IncMargin{1em}
%\lipsum[1-2]

\begin{algorithm}
\ssmall
 \caption{RECS Algorithm}
 \ssmall
\label{Algorithm:1}
\SetKwData{Left}{left}\SetKwData{This}{this}\SetKwData{Up}{up}\SetKwFunction{Union}{Union}\SetKwFunction{FindCompress}{FindCompress}\SetKwInOut{Input}{Input}\SetKwInOut{Output}{Output}
\algsetup{linenosize=\tiny}
\begin{minipage}{.5\textwidth}

\Algphase{a: Neighborhood Expansion}
\SetAlgoLined

\Input{Graph $G(V,E)$ \\
       $u$: node to expand \\
      $e$ $(default: 1200)$ %size of neighborhood expansion subgraph
      }
      
\Output{$N_E(u)$}
    
    Add node $z$ to $G(V,E)$\

    Connect $V$ (except $u$ and $z$) to $z$\

    Initialize $EX=\{u\}$\
    
    Initialize $P=\{v_1,v_2, ... ,v_n\}$ (neighbors of $u$)\

\While { $|EX| <$ $(default: 1200)$}{

minDistance = infinity\ 

\For{$p \in P$}{
    
    newDistance =  Compute Distance($u,p$)\
    
    \If{minDistance $>$ newDistance}
    { minDistance = minDistance}
}     

    Add node(minDistance) to $EX$\ 
    
    Remove node(minDistance) from $P$\
    
    Add neighbors of node(minDistance) to $P$\
    
}

Remove node $z$ from $G(V,E)$

return subgraph $(EX, G(V,E))$\ 
           \hfill \break

\end{minipage}%
\begin{minipage}{.5\textwidth}

\Algphase{b: Neighborhood Refinement}
\SetAlgoLined

\Input{$N_E(u)$ \\
      $r$ $(default: 800)$ %: size of neighborhood expansion subgraph\\
      \\
      $u:$ node to refine\\
      }
\Output{$N_R(u)$ }

Add node $z$ to graph N_E(u)\

Connect all nodes in graph N_E(u) (except $u$ and $z$) to  $z$\

Initialize voltageOf$[u] = 1$ and voltageOf$[z] = 0$\

Initialize $N_R$ = \{ \}

Calculate Voltage and Current for each node in $(N_E(u))$

    
\While{ $|N_R(u)| <$ $(default: 800)$}{

 Add all nodes along the path that maximizes the current between $u$ and $z$ to $N_R$
                
}

return subgraph($N_R$, $N_E(u)$ )\ 

\
\
\
\
\
\



\end{minipage}


\end{algorithm}

\vspace{0.15cm}

After we compute the voltages for each node in an \textit{expanded} subgraph, we calculate the currents of each edge in the subgraph using Ohm's law. Most importantly, current computations must satisfy downhill constraint. Thus, we need to sort subgraph's nodes in a descending order, based on their calculated voltage values. Using computed currents of the \textit{expanded neighborhood} subgraph, we form the \textit{refined neighborhood} subgraph, which represents node's neighborhood. The way in which we creat \textit{refined neighborhood} subgraph is by adding end-to-end paths from node $z$ to node $u$ one at a time, until we reach the predetermined \textit{refined} subgraph size, $|N_R(u)|$. It is important to note that each time we add a path to the \textit{refined} subgraph, we add the nodes that are not already included in the subgraph. Therefore, we use dynamic programming to implement our \textit{refinement} process, which is like a depth first search (DFS) approach with a slight modification. We always start from node $z$. For traversing, we traverse neighbors in a descending order of current ($I$) reached to the node we are visiting from the neighboring nodes. In addition, we add each node we visit to the \textit{refinement} subgraph. For tracing back, we traceback when we visit all neighboring nodes or when we reach node $u$. Our way in identifying node neighborhoods is more concrete and rational comparing to representation learning baseline algorithms for the following reasons: 1) We preserve the local and global structure of network by accounting for the immediate neighbors and neighbors at increasing distances of the source node $u$ to identify its neighborhood; 2) We generate neighborhoods on distance and network flow bases; 3) We address the issue of high-node degree distribution; 4) We concurrently identify neighborhood notions while maximizing proximity among non-adjacent nodes, which are abundant in real-world networks; and 5) We design our algorithm such that it yields consistent stable representations that suite single and multiple graph problems.       

\subsection{Step 2: Representation Vector Update} 
\label{subsec:step2}

After identifying node neighborhoods in a graph, we aim to learn node representations. For that, we adopt SkipGram model~\cite{mikolov2013efficient} to learn node representations by optimizing the following objective. This objective maximizes the log-probability of observing the pre-identified neighborhood generated via \textit{refinement} phase; $N_R(u_i)$, for the node $u_i$ given its feature representations provided by \textit{f}:

\begin{equation} \label{eq:7}
\ssmall
\underset{f}{\text{max}}\sum_{u\in V}\log(Pr(N_R(u)\mid f(u))
\end{equation}

In order to make the maximum likelihood optimization problem tractable, here we list two assumptions must be satisfied:\\

\noindent \textbf{Assumption 1 -- Conditional independence.} Here we assume that the likelihood of observing any node neighborhood notion is completely independent of observing any other node neighborhood notion given the feature representation of the given node of interest $u$:

\begin{equation} \label{eq:8}
\ssmall
Pr(N_R(u)\mid f(u))=\prod_{n_i\in N_R(u)}Pr(n_i\mid f(u)) 
\end{equation}
where $n_i$ represents any node that belongs to node $u$'s refined neighborhood notion.\\

\noindent \textbf{Assumption 2 -- Symmetry in feature space.} The source node $u$ and any other node belongs to its refined neighborhood notion $(n_i)$, have a symmetrical impact over each other in the continuous feature space. Therefore, the conditional probability, $Pr(n_i \mid u)$, is modeled using the softmax function as follows:

\begin{equation} \label{eq:9}
\ssmall
Pr(n_i\mid f(u)) =\frac{\exp(f(n_i)\cdot f(u))}{\sum_{v\in V}\exp(f(v)\cdot f(u))}
\end{equation}

Based on the above two assumptions, we can simplify the objective in Eq.\eqref{eq:7} as follows:

\begin{equation} \label{eq:10}
\ssmall
\underset{f}{\text{max}}\sum_{u\in V}\bigg[-\log\sum_{v\in V}\exp(f(v)\cdot f(u))+\sum_{n_i\in N_R(u)}f(n_i)\cdot f(u)\bigg]
\end{equation}

It is important to note that performing such calculations for each node in large-scale graphs is computationally expensive. Therefore, we here approximate the function using negative sampling~\cite{mikolov2013distributed}. We optimize objective shown in Eq.\ref{eq:10} using stochastic gradient decent.

\subsection{Illustrative Example}
We here make-up an illustrative example, so that it would be easier to follow and understand performed computations. This example describes identifying node neighborhoods two steps in detail as follows:\\

\noindent \textbf{Phase A: Neighborhood Expansion - $N_E(u)$.} Figure~\ref{fig:step1} shows the details of generating $N_E(u)$. The given graph $G$ is an undirected and unweighted graph. We assume the conductance of real existing edges---i.e., edges not connecting with node $z$--- $=1$. We set $e=5$, so that we stop when we have five nodes in $N_E(u)$. In order to compute conductance values of edges connecting nodes $1-56 $ with node $z$, we employ Eq.\eqref{eq:1}. We assume $\alpha=1$. The computed conductance values are shown on the red-dotted edges, as shown in in Figure~\ref{fig:step1}-a. After the conductance computations, we compute the distances between node $u$ and the remaining nodes $1-56$ using Eqs.~\eqref{eq:2} and~\eqref{eq:3}. Table~\ref{my-label3} shows the values of the computed distances. As shown in Figure~\ref{fig:step1}(b-e), we expand node $u$'s neighborhood by gradually adding nodes $1, 2, 3$ and $51$, respectively, on distance basis. Since we assume $e=5$, we stop the expansion after including the four closest nodes to node $u$. 

\begin{figure}[t!]
\includegraphics[width=0.8\textwidth]{Figures/Step1.png}
\centering
\setlength{\abovecaptionskip}{15pt plus 3pt minus 2pt}
\caption{The illustrative example expansion step of node $u$. (a): Represents the given graph, $G$. The numbers on the red-dotted edges represent the conductance values of edges connecting nodes $1$-$56$ with node $z$. (b-e): Represent the expansion process. To expand node $u$, nodes $1, 2, 3,$ and $51$ are added, respectively, on a distance basis. The closer the neighbor to node, $u$, the higher the probability it has to be added to $N_E(u)$.}
\label{fig:step1}
\vspace{-0.5cm}
\end{figure}

\begin{table}[t!]
\ssmall
\parbox{.45\linewidth}{
\centering
\caption{Distances between node $u$ and the remaining nodes; $1$-$56$.}
\label{my-label3}
\begin{tabular}{@{}lc@{}}
\toprule
Node Pair       & $Distance (D)$ \\ \midrule
$(u,1)$           & $0.95$         \\
$(u,2)$           & $0.95$         \\
$(u,3)$           & $0.95$         \\
$(u,4) - (u,50)$  & $4.91$         \\
$(u,51)$          & $2.51$         \\
$(u,52)$          & $2.51$         \\
$(u,53) - (u,56)$ & $2.95$         \\ \bottomrule
\end{tabular}
}
~~~~~~~~~\parbox{.45\linewidth}{
\centering
\caption{Total currents flow in paths connecting nodes $u$ and $z$ in $N_E(u)$ \vspace{0.65cm}}
\label{my-label4}
\begin{tabular}{@{}lc@{}}
\toprule
Path  & Total Current \\ \midrule
$u$\rightarrow{$1$}\rightarrow{$z$}   & 1.94          \\
$u$\rightarrow{$2$}\rightarrow{$z$}   & 1.44          \\
$u$\rightarrow{$3$}\rightarrow{$z$}   & 1.68          \\
$u$\rightarrow{$2$}\rightarrow{$51$}\rightarrow{$z$} & 1.00          \\ \bottomrule
\end{tabular}
}
\end{table}


\noindent \textbf{Phase B: Neighborhood Refinement - $N_R(u)$.} After we expand node $u$ on a distance basis, we need to further prune out the generated subgraph, but this time, on a current basis. Therefore, we need to first compute the voltage for each node in the expanded subgraph; $N_E(u)$, using Eq.\eqref{eq:5}. We compute node voltage values by solving the system of the linear equations under the boundary conditions shown in Eq.\eqref{eq:6}. In Eq.\eqref{eq:11}, we show the voltage computation of node $1$. The same applies to nodes $2, 3,$ and $51$.

\begin{equation} \label{eq:11}
\ssmall
V(1)=\frac{V(u)(1)+V(z)(48)}{1+48}
\end{equation}

%\begin{equation} \label{eq:12}
%\small
%V(2)=\frac{V(u)(1)+V(z)(3)+V(51)(1)}{1+3+1}
%\end{equation}

%\begin{equation} \label{eq:13}
%\small
%V(3)=\frac{V(u)(1)+V(z)(5)}{1+5}
%\end{equation}

%\begin{equation} \label{eq:14}
%\small
%V(51)=\frac{V(2)(1)+V(z)(1)}{1+1}
%\end{equation}

Now, after we compute the node voltage values, we need to compute the current flows on each edge connecting any two immediate nodes in $N_E(u)$. However, based on Ohm's law shown in Eq.\eqref{eq:4}, in order for a current to flow from node $n_1$ to node $n_2$, we need node $n_1$ to have a higher voltage than node $n_2$, which is defied as the downhill constraint. Therefore, we need to sort the $N_E(u)$ nodes in a descending order based on their voltage values. Figure~\ref{fig:step2}-b shows the directions in which currents flow between each two immediate nodes. The current flows from the node of higher voltage to the node of lower voltage---i.e., current flows from node $2$ to node $51$. Using the computed voltage values, we compute currents using Eq.\eqref{eq:4}. The values of the computed currents are shown on the red-dotted edges on Figure~\ref{fig:step2}-b. 

After computing the currents values, we find all possible paths between nodes $u$ and $z$ (shown in Table~\ref{my-label4}). For each path, we compute the total current flows between nodes $u$ and $z$ by adding the current of each edge along the path. Total current value for each path is shown in Table~\ref{my-label4}. Now, we sort the paths in a descending order of their total current values. Finally, we add path by path to the refinement subgraph and check the size of refinement subgraph after each addition to see if we have meet the stopping criteria ($|N_R(u)| => r$).
%traceback from node $z$ to node $u$ by adding one path at a time, which maximizes the current delivered to node $z$ from node $u$. Figure~\ref{fig:step2}-b shows that node $z$ receives currents from nodes $1, 2, 3$ and $51$. The maximum received current $=0.96$ and is from node $1$. Therefore, we visit node 1 and since node 1 receives current only from node $u$ then we visit node $u$. Since node $u$ is the end of the path, we have found the first path that deliver the maximum current to node $z$ from node $u$, which is $z$->1->$u$. Thus, we add nodes 1 and $u$ to $N_R$}. We now check if we have met the stopping criteria ($|N_R(u)|==3$) and since |$N_R$| < 3, we need to continue and add one more path. Therefore, we mark node $u$ as visited and traceback to node 1. Since we visited all paths that node 1 received current from we tracback to node $z$. Now, we did not visit  all paths that 
Since we assume $r=3$, we stop when we have at least three nodes in $N_R(u)$. The generated $N_R(u)$'s are then fed into the SkupGram model to learn node representations.

\begin{figure}[t!]
\includegraphics[width=0.8\textwidth]{Figures/Step2.png}
\centering
\setlength{\abovecaptionskip}{15pt plus 3pt minus 2pt}
\caption{The illustrative example refinement step of node $u$. (a): Shows the expanded subgraph, $N_R(u)$, generated by the previous expansion step. The numbers on the red-dotted edges represent the edge conductance values of nodes $1, 2, 3$, and $51$ with node $z$. (b): Shows the computed node voltage values inside the nodes, and the computed currents on the red-dotted and black-solid edges. (c): Shows the addition of the first path connecting node $u$ and node $1$. (d): Shows the addition of the second path connecting node $u$ and node $3$. It also represents the generated $N_R(u)$.}
\label{fig:step2}
\end{figure}
